MaskSearch: Querying Image Masks at Scale

Machine learning tasks over image databases often generate masks that annotate image content (e.g., saliency maps, segmentation maps, depth maps) and enable a variety of applications (e.g., determine if a model is learning spurious correlations or if an image was maliciously modified to mislead a model). While queries that retrieve examples based on mask properties are valuable to practitioners, existing systems do not support them efficiently. In this paper, we formalize the problem and propose MaskSearch, a system that focuses on accelerating queries over databases of image masks while guaranteeing the correctness of query results. MaskSearch leverages a novel indexing technique and an efficient filter-verification query execution framework. Experiments with our prototype show that MaskSearch, using indexes approximately 5% of the compressed data size, accelerates individual queries by up to two orders of magnitude and consistently outperforms existing methods on various multi-query workloads that simulate dataset exploration and analysis processes.

==> optimization.tex <==
\section{Optimizations}

In this section, we discuss the optimizations that we have made to the query execution algorithm to improve its performance.


\subsection{Maintaining Sort Order} \label{sec:sort-order}

Sort order is useful when computing the upper bound and lower bound in the filter step (instead of loading the masks from disk in the verification step) becomes the bottleneck of the query execution with all the techniques discussed above.


\subsection{Multi-Query Caching}

\subsection{Index Compression}
Use run-length encoding to compress the index across grids.

\subsection{Approximate Query Processing}
